Model and Machine Learning based Caching and Routing Algorithms for Cache-enabled Networks

In-network caching is likely to become an integral part of various networked systems (e.g., 5G networks, LPWAN and IoT systems) in the near future. In this paper, we compare and contrast model-based and machine learning approaches for designing caching and routing strategies to improve cache network performance (e.g., delay, hit rate). We first outline the key principles used in the design of model-based strategies and discuss the analytical results and bounds obtained for these approaches. By conducting experiments on real-world traces and networks, we identify the interplay between content popularity skewness and request stream correlation as an important factor affecting cache performance. With respect to routing, we show that the main factors impacting performance are alternate path routing and content search. We then discuss the applicability of multiple machine learning models, specifically reinforcement learning, deep learning, transfer learning and probabilistic graphical models for the caching and routing problem.

==> algo.tex <==




==> biography.tex <==
%\vspace{-17 cm}
\vspace{-10 cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{anand}}]{Anand Seetharam}
is an assistant professor in the computer science department at State University of New York Binghamton. He obtained his PhD. from University of Massachusetts Amherst in 2014. He is broadly interested in the field of computer networking. His research encompasses  internet-of-things, information-centric networks, wireless networks, and security. He has published numerous papers in peer-reviewed journals and conferences. 
\end{IEEEbiography}

\vspace{-11 cm}
\begin{IEEEbiography}[{ \vspace{- 1cm} \includegraphics[width=1in,height=1in,clip,keepaspectratio]{adita}}]{Adita Kulkarni} is a graduate student in the Computer Science department at SUNY Binghamton. She received her Bachelor of Engineering degree in Computer Engineering from Savitribai Phule Pune University, India. Her research interests include information-centric networks, mobile computing and wireless systems.
\end{IEEEbiography}






==> broaderimpact.tex <==
The proposed research takes an important step forward in addressing the pressing challenges in the area of cyber-physical systems. If successful, the proposed research will advance the state-of-the-art, and take a significant stride in realizing a smarter community. Results of our research will be disseminated through publications at peer-reviewed conferences and journals. The PIs plan to organize workshops related to smart computing and smart grids that provide a shared platform for researchers in the area of machine learning, networking and cyber-physical systems to engage in research discussions. 

\noindent {\bf Diversity:} Graduate research assistants in the Computer Science Department at Binghamton University and UMass Amherst will be actively involved in this project. At Binghamton University, the research will be primarily accomplished by PI Seetharam and his female PhD student Yasra Chandio, working with the PI on her PhD in the area of smart cities and smart grids, and PI Ramesh and Gissella Bejarano, a female Hispanic PhD student working on designing deep learning models for smart computing applications. Both PI Seetharam and PI Ramesh have  made an active effort in recruiting and mentoring female graduate students and each of them has two female PhD students working with them. As a member of the ACM Future of Computing Academy, PI Seetharam is involved in working groups that seek to improve the participation of underrepresented communities in computer science. 
{\bf At University of Massachusetts Amherst - \red{TODO} for Prashant.}

\noindent {\bf Undergraduate Mentoring:} The project also has smaller tasks suitable for undergraduate students. They will be assigned tasks such as parsing and cleaning the publicly available traces so that they can used for testing the proposed  algorithms and models. Similarly, undergraduate students will be employed in setting up the testbed as well as testing and maintaining its different components. We plan to seek supplementary REU funding to involve additional undergraduate researchers into this project. PI Ramesh has an established record of  successfully working with undergraduate students and David Defazio, an undergraduate student working with her was awarded the top undergraduate researcher at a University wide research competition.{\bf \red{TODO} - We need to discuss and budget for this.}

\noindent {\bf Education Plan:} Since joining Binghamton University, PI Seetharam and PI Ramesh have organized a joint reading group for graduate students on advanced topics in the area of systems and machine learning. The reading group was well received and we plan to continue this effort. The PIs also plan to co-teach a new course on cyber-physical systems that will be offered jointly at UMass Amherst and Binghamton University. The course will include presentations from students at both locations and will provide students the opportunity to collaborate on research projects with students located at the other campus. All teaching materials for this course including a full set of course slides, and homework will be made available online, so that faculty at other universities can use them. 

{\bf About PI Shenoy  - \red{TODO} for Prashant.}

\noindent {\bf Anything Else:} {\bf \red{TODO} - Community outreach, testbed implementation in community?}


==> contributions.tex <==
In this section, we  first outline our proposed research on designing control decision algorithms for the home-level and grid-level optimization problems. As the control decision algorithms  rely heavily on predicted future solar energy generation and home energy consumption, we propose deep learning models to generate these predictions. We also propose an iterative algorithm that executes periodically in an online manner to improve the quality of these predictions.


\subsection{Designing Control Decision Algorithms} 
\input{algo}
\label{sec:algo}


\subsection{\red{TODO} Deep Learning Models for Solar Energy Generation and Home Energy Consumption} 
\input{op-coop}
\label{sec:deep}

==> objectives.tex <==
\vspace{- 1cm}
\noindent {\bf Objective:} The main objectives of this proposal are to
\begin{itemize}
\item{Design caching algorithms for  wireless cache networks that  take into account factors such as content popularity, wireless channel quality, interference, network connectivity and mobility  to maximize  network-level (e.g., hit rate) and user-level (e.g., delay, throughput) performance. }
\item{ Analytically model the performance of opportunistic and cooperative forwarding strategies in multi-hop wireless cache networks considering uncorrelated and correlated wireless channel models, and in the presence of multiple competing and interfering flows.}
\item{Evaluate the proposed algorithms and validate the analytical results on real-world traces, and in mobile scenarios.}
\end{itemize}


==> prior.tex <==
PIs Seetharam and Ramesh do not have any prior NSF support.

==> timeline.tex <==
%!TEX root = main.tex
In this section, we outline our project management and collaboration plan to achieve the proposed objectives. The PIs will hold weekly online meetings  to discuss the progress of the project. To foster collaboration, the PIs will also meet face-to-face at least twice each semester at UMass Amherst or at  Binghamton University. Additionally, graduate students will visit either university regularly to facilitate knowledge transfer and discuss research ideas.

%Figure \ref{} shows how the PIs plan to collaborate to achieve the proposed objectives. 

\noindent {\bf Year 1:} {\it Control Decision Algorithms:} PI Seetharam and PI Shenoy will work with their students to design the control decision algorithms for the home and grid-level problems. As a first step, we will design algorithms that have complete knowledge of future home energy consumption and solar energy generation, and test them on publicly available traces. This analysis will help us determine the upper bound on the performance of our algorithms.\\
{\it Deep Learning Models:} PI Ramesh and her students will focus on developing the deep learning models for home energy consumption and solar energy generation and investigate the performance of these models via trace-based evaluation. PI Shenoy will provide the domain expertise needed to design these deep models.\\ %which are part of the deep latent models
{\it Prototype Testbed:} In collaboration with PI Shenoy, PI Seetharam will set up a testbed similar to the one at UMass Amherst at Binghamton University. We plan to have a basic functional testbed setup at Binghamton University by the end of  this year.

\noindent {\bf Year 2:} {\it Control Decision Algorithms:} PI Seetharam  and PI Shenoy will work with their students to integrate predictions generated by the deep learning models and the insights learned by the latent variables in year 1 in the control decision algorithms and test them via trace-based evaluation. \\
{\it Deep Learning Models:} PI Ramesh and her  students will focus on integrating the deep generative models with discriminative models and develop the online backpropogation algorithm to update the predictions periodically.\\
{\it Prototype Testbed:} PI Shenoy and PI Seetharam will continue to work on the testbed. We plan to have a fully functional testbed setup at Binghamton University by the end of this year. 

\noindent {\bf Year 3:}  {\it Control Decision Algorithms:} PI Seetharam  and PI Shenoy along with their students will work on integrating the updated predictions provided by the online algorithm in the control decision algorithms. We plan to test the proposed algorithms on data generated from the testbed and also conduct the factor analysis described in Section \ref{sec:factoranalysis}.\\
{\it Deep Learning Models:} PI Ramesh will work with PIs Seetharam and Shenoy and focus on using the feedback (in terms of performance) obtained   from the control decision algorithms to improve the deep learning models. A thorough evaluation of the deep learning models, data augmentation and the online algorithm will be conducted by using data  collected from multiple testbeds and publicly available traces. \\
{\it Prototype Testbed:}  As we plan to generate significant data from the testbeds during this year, we will take steps for data preservation and making it readily accessible. We will also implement the control algorithms on the testbeds to demonstrate their feasibility in real-world settings.


% on data augmentation and improvements achieved by the o on the testbed and

%The control decision algorithms will be iteratively improved by considering both deep latent models and the online algorithm for updating predictions.
%will be  improved by incorporating the feedback from the control decision algorithm in the deep latent models and vice versa.\\

%
%\noindent 
%
%In collaboration with PI Shenoy, PI Seetharam will set up a testbed similar to the one at University of Massachusetts Amherst at Binghamton University. We plan to have a basic functional testbed setup at Binghamton University at the end of Year 1.
%
%\noindent {\bf Year 2:}  PI Seetharam and PI Ramesh will work on designing the algorithms and models for predicting future household energy consumption and renewable energy generation. Along with PI Shenoy, they will work on testing these algorithms on publicly available traces as well as traces generated from the testbed at University of Massachusetts Amherst. 
%
%\noindent  PI Ramesh and PI Shenoy will work on completing the design of the proposed deep learning framework. Some preliminary results will also be generated based on publicly available traces. 
%
%\noindent We expect the testbed design to be completed by this year and initial data needed to achieve Objective 2 will be collected. The PIs will also work on incorporating the algorithms designed for Objective 1 into the real test bed
%
%\noindent {{\bf Year 3:} We believe that most research related to these objectives would have been accomplished by the third year.
%
%\noindent  We plan exhaustive test and validate the algorithms designed for objectives 1 and 2 during this year. Specifically, with respect to Objective 1, our goal will be to demonstrate the feasibility and benefits obtained via a real-world prototype. With respect to Objective 2, we note that to ensure that we will ?? The research results obtained will also be submitted to peer-reviewed conferences and journals during this year.

